Niche Dynamics in Complex Online Community Ecosystems

Online communities are important organizational forms where members socialize and share information. Curiously, different online communities often overlap considerably in topic and membership. Recent research has investigated competition and mutualism among overlapping online communities through the lens of organizational ecology; however, it has not accounted for how the nonlinear dynamics of online attention may lead to episodic competition and mutualism. Neither has it explored the origins of competition and mutualism in the processes by which online communities select or adapt to their niches. This paper presents a large-scale study of 8,806 Reddit communities belonging to 1,919 clusters of high user overlap over a 5-year period. The method uses nonlinear time series methods to infer bursty, often short-lived ecological dynamics. Results reveal that mutualism episodes are longer lived and slightly more frequent than competition episodes. Next, it tests whether online communities find their niches by specializing to avoid competition using panel regression models. It finds that competitive ecological interactions lead to decreasing topic and user overlaps; however, changes that decrease such niche overlaps do not lead to mutualism. The discussion proposes that future designs may enable online community ecosystem management by informing online community leaders to organize "spin-off" communities or via feeds and recommendations.

==> methods_flowchart.tex <==
 
\tikzset{
  observed/.style={circle, draw},
  partly observed/.style 2 args={draw, fill=#2, path picture={
      \fill[#1, sharp corners] (path picture bounding box.south west) -|
      (path picture bounding box.north east) -- cycle;},
     circle},
    unobserved/.style={draw, circle, fill=gray!30},
    residual/.style={draw, rectangle},
    data/.style={draw, rectangle, fill=white,inner sep=0.1in, align=left,rounded corners=0.5em, anchor=south west, align=center, execute at begin node=\setlength{\baselineskip}{1em}},
       selection_data/.style={draw, rectangle, style=densely dashdotted,    rounded corners = 0.5em,align=center,
 fill=white,inner sep=0.1in, align=left, anchor=south west, execute at begin node=\setlength{\baselineskip}{4ex}},
    decision box/.style={draw, diamond, fill=blue!20, text width=2in, align=center, inner sep=0.1in, anchor=south west, execute at begin node=\setlength{\baselineskip}{1ex},aspect=3},
    process/.style={draw, rectangle, fill=gray!5, text width=2in, inner sep=0.25in, align=center, anchor=south west, execute at begin node=\setlength{\baselineskip}{4ex}},
        show curve controls/.style={
    postaction={
      decoration={
        show path construction,
        curveto code={
          \draw [blue] 
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentsupporta)
            (\tikzinputsegmentlast) -- (\tikzinputsegmentsupportb);
          \fill [red, opacity=0.5] 
            (\tikzinputsegmentsupporta) circle [radius=.2ex]
            (\tikzinputsegmentsupportb) circle [radius=.2ex];
        }
      },
      decorate
    }},
    myarrow/.style={
    arrows={-Stealth[round]},
    scale=1,
  },
  selection_arrow/.style={
    arrows={-Stealth[round]},
    scale=1,
    style=densely dashdotted,
    },
    myarrownotip/.style={
    scale=1,
    line width=1pt
    },
    mylabel/.style={
      text width=2.2in,
      text=gray!90,
      align=center,
      execute at begin node =\setlength{\baselineskip}{1.3ex},
      inner sep=1ex,
      font={\bfseries\itshape\sffamily #1}
    },
    myframe/.style={
      line width=0.7pt, draw=gray!60, inner ysep=0.5em, inner xsep=0.9em},
}
\newcommand{\myindent}{\hspace{1em}}

\begin{tikzpicture}[every node/.style={transform shape}, scale=0.775]

  \node[data](pushshift_reddit)[text width=1.7in] {Reddit posts \& comments};

  \node[data](phrases)[right of=pushshift_reddit,xshift=2.2in] {Detected phrases};
  \node[data](accounts)[below of=phrases, yshift=-1em] {Posts \& comments \\ by  account};

  % \node[data](phrase_tfidf)[right of=pushshift_reddit, xshift=2in] {Phrases tfidf};

  % \node[data](author_tfidf)[below of=phrase_tfidf] {Authors tfidf};

 
  \node[selection_data](phrase_lsa_model)[right of=phrases, xshift=1.6in] {Topic LSA model}; 

  \node[selection_data](author_lsa_model)[below of=phrase_lsa_model,yshift=-1em] {User LSA model}; 

% add nodes for "LSA models" that connect to the similarity time series.
  \node[selection_data](phrase_lsa)[right of=phrase_lsa_model, xshift=10em] {Topic overlap}; 

  \node[selection_data](author_lsa)[below of=phrase_lsa,yshift=-1em] {User overlap}; 


  \node[selection_data](hdbscan_authors) [below of=author_lsa,yshift=-5em, xshift=-6em] {User clusters};

  \node[selection_data](hdbscan_phrases)[above of=hdbscan_authors] {Topic clusters};

  \node[data](active_author_timeseries)[below of=pushshift_reddit,yshift=-4em, text width=1.5in] {Posts \& comments by account each week};

  \node[data](smap_jacobians)[below of=active_author_timeseries,yshift=-4em, text width=1.5in] {Competition-mutualism over time (H1)};

  \node[data](phrase_weekly_lsa)[below of=accounts, yshift=-3em, xshift=-2.25em] {Topic overlap over time}; 

  \node[data](author_weekly_lsa)[below of=phrase_weekly_lsa, yshift=-1em] {User overlap over time}; 


  \node[data](preg)[below of=author_weekly_lsa, yshift=-4em]{Panel regression models (H2,H3)};

  % create a frame labeled "model selection" around phrase_lsa, author_lsa, topic_clusters, author_clusters. 

\draw[selection_arrow] (hdbscan_phrases.110) to [controls=+(0:0) and +(320:1)]  (phrase_lsa_model.355){};

\draw[selection_arrow] (hdbscan_authors.190) to [controls=+(190:0.5) and +(290:1)]  (author_lsa_model.260){};

  \node[color=black, mylabel, draw,  style=densely dashdotted, below of=hdbscan_authors, text width=3in, yshift=-2.5em](model_selection){Model selection \\ for Latent Semantic Analysis (LSA) \\
    (TF-IDF $\rightarrow$ SVD)};
 %\node[myframe,fit=(phrase_lsa_model)(author_lsa_model)(phrase_lsa)(author_lsa)(hdbscan_phrases)(hdbscan_authors)]{};


\draw[myarrow] (pushshift_reddit) to (phrases) {node [mylabel, xshift=-1.1in, yshift=2.2em, text width=1in] {Pointwise mutual information (10\% sample) }};

\draw[myarrow] (phrases) to (phrase_lsa_model);
\draw[myarrow] (accounts) to (author_lsa_model);

\draw[selection_arrow] (phrase_lsa_model) to (phrase_lsa);
\draw[selection_arrow] (author_lsa_model) to (author_lsa);


\draw[myarrow] (pushshift_reddit.340) to [controls=+(330:1.3) and +(180:0.5)] (accounts.west);
 
 
\draw[selection_arrow] (author_lsa) to [controls=+(330:1) and +(10:0.7)](hdbscan_authors.east);
\draw[selection_arrow] (phrase_lsa.350) to [controls=+(310:2) and +(10:1.7)] (hdbscan_phrases.350) {node [mylabel, xshift=0.65in, yshift=-1.7em] {HDBSCAN \\ clustering}};
\draw[myarrow] (pushshift_reddit) to (active_author_timeseries);

\draw[myarrow] (hdbscan_authors) to (author_weekly_lsa);
\draw[myarrow] (hdbscan_authors) to (phrase_weekly_lsa);
\draw[myarrow] (active_author_timeseries) to (smap_jacobians) {node [mylabel, xshift=-5em, yshift=3.5em] {Regularized SMAP}};
\draw[myarrow] (active_author_timeseries) to (author_weekly_lsa.west);
% \draw[myarrow] (phrases.190) to [controls=+(190:2.2) and +(170:0.8)] (phrase_weekly_lsa.172);
\draw[myarrow] (active_author_timeseries.355) to [controls=+(355:0.3) and +(180:0.7)](phrase_weekly_lsa.182);
\draw[myarrow] (smap_jacobians) to (preg);
\draw[myarrow] (phrase_weekly_lsa.east) to [controls=+(355:4) and +(35:2.5)] (preg);
\draw[myarrow] (author_weekly_lsa) to (preg);

\draw[myarrow] (author_lsa_model.195) to [controls=+(190:0.8) and +(15:1.2)] (author_weekly_lsa.8);
\draw[myarrow] (phrase_lsa_model.195) to [controls=+(190:0.8) and +(15:1.2)] (phrase_weekly_lsa.8);
\draw[myarrow] (hdbscan_authors.200) to [controls=+(200:0.8) and +(350:4.5)] (smap_jacobians.350);


\end{tikzpicture}


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "paper.Rtex"
%%% End:

